Naive Automated Machine Learning -- A Late Baseline for AutoML

Automated Machine Learning (AutoML) is the problem of automatically finding the pipeline with the best generalization performance on some given dataset. AutoML has received enormous attention in the last decade and has been addressed with sophisticated black-box optimization techniques such as Bayesian Optimization, Grammar-Based Genetic Algorithms, and tree search algorithms. In contrast to those approaches, we present Naive AutoML, a very simple solution to AutoML that exploits important meta-knowledge about machine learning problems and makes simplifying, yet, effective assumptions to quickly come to high-quality solutions. While Naive AutoML can be considered a baseline for the highly sophisticated black-box solvers, we empirically show that those solvers are not able to outperform Naive AutoML; sometimes the contrary is true. On the other hand, Naive AutoML comes with strong advantages such as interpretability and flexibility and poses a strong challenge to current tools.

==> candidate-evaluations.tex <==
\subsubsection{Candidate Evaluations}
\label{sec:candidateevalution}
To assess the performance of a candidate we construct empirical learning curves for it.
To this end, starting from a sample with a small number of instances, we successively evaluate its validation performance after being fitted on a growing number of instances.
We refer to the training sizes on which candidates are evaluated as \emph{anchor points}.
At each anchor point $t$, the candidate is evaluated not only once but a repeated number of times to obtain more stable estimates.

The evaluation procedure for the candidates has two important advantages over conducting a kind of cross-validation of the candidates on the full data.
First, if the candidate would time out on the full data but can be built successfully on smaller data portions, we obtain an estimate at all instead of a failure.
Second, instead of only the estimate of a single point in the learning curve, we obtain a \emph{series} of estimates of different points, which allows us to make a qualified guess on the potential improvement of the classifier on more data.

Based on the anchor points, we can derive a learning curve of the candidate and, under the assumption of learning curve convexity, leverage it for predicting the loss for larger samples of the dataset.
The interpolation is done by observing the minimum slope between any two anchor points and assuming this slope for the remaining learning curve up to the point of interest.
Thereby, we can estimate a \textit{bound} on the best possible performance that can be expected on the number of training examples that will be decisive for the ordering of candidates.
Note that estimating a valid bound is much easier than estimating the true performance at some anchor point as done in learning curve prediction \cite{}.

Such a bound can then be used to stop a pipeline evaluation early.
Let $n$ be the overall number of instances available for training, and let $\hat{z}$ denote the estimated performance when training on $n$ instances obtained from the learning curve extrapolated to the point $n$.
Furthermore, let $z^\ast$ denote the performance of the best actually observed performance among all candidates on $n$ instances.
Assuming hyper-parameter optimization to improve the performance by $\varepsilon$ and admitting an error $\xi$ in the bound estimate, we can discard a candidate if
$$\hat{z} > z^\ast + \varepsilon + \xi \, .$$
Therefore, a candidate is discarded if the performance $\hat{z}$ when being trained on $n$ instances cannot be expected to be competitive with the best performance $z^\ast$ already observed.

==> header.tex <==
\twocolumn[
\icmltitle{Naive Automated Machine Learning: A Late Baseline for AutoML}

% It is OKAY to include author information, even for blind
% submissions: the style file will automatically remove it for you
% unless you've provided the [accepted] option to the icml2021
% package.

% List of affiliations: The first argument should be a (short)
% identifier you will use later to specify author affiliations
% Academic affiliations should list Department, University, City, Region, Country
% Industry affiliations should list Company, City, Region, Country

% You can specify symbols, otherwise they are numbered in order.
% Ideally, you should not use this facility. Affiliations will be numbered
% in order of appearance and this is the preferred way.
\icmlsetsymbol{equal}{*}

\begin{icmlauthorlist}
\icmlauthor{Aeiau Zzzz}{equal,to}
\icmlauthor{Bauiu C.~Yyyy}{equal,to,goo}
\icmlauthor{Cieua Vvvvv}{goo}
\icmlauthor{Iaesut Saoeu}{ed}
\icmlauthor{Fiuea Rrrr}{to}
\icmlauthor{Tateu H.~Yasehe}{ed,to,goo}
\icmlauthor{Aaoeu Iasoh}{goo}
\icmlauthor{Buiui Eueu}{ed}
\icmlauthor{Aeuia Zzzz}{ed}
\icmlauthor{Bieea C.~Yyyy}{to,goo}
\icmlauthor{Teoau Xxxx}{ed}
\icmlauthor{Eee Pppp}{ed}
\end{icmlauthorlist}

\icmlaffiliation{to}{Department of Computation, University of Torontoland, Torontoland, Canada}
\icmlaffiliation{goo}{Googol ShallowMind, New London, Michigan, USA}
\icmlaffiliation{ed}{School of Computation, University of Edenborrow, Edenborrow, United Kingdom}

\icmlcorrespondingauthor{Cieua Vvvvv}{c.vvvvv@googol.com}
\icmlcorrespondingauthor{Eee Pppp}{ep@eden.co.uk}

% You may provide any keywords that you
% find helpful for describing your paper; these are used to populate
% the "keywords" metadata in the PDF but will not be shown in the document
\icmlkeywords{Machine Learning, ICML}

\vskip 0.3in
]

% this must go after the closing bracket ] following \twocolumn[ ...

% This command actually creates the footnote in the first column
% listing the affiliations and the copyright notice.
% The command takes one argument, which is text to display at the start of the footnote.
% The \icmlEqualContribution command is standard text for equal contribution.
% Remove it (just {}) if you do not need this facility.

%\printAffiliationsAndNotice{}  % leave blank if no need to mention equal contribution
\printAffiliationsAndNotice{\icmlEqualContribution} % otherwise use the standard text.

==> results.tex <==
\begin{tabular}{rrr}
\toprule
 openmlid &                                                      naive &                                                     mlplan \\
\midrule
        3 &   \underline{0.0069$\pm$0.0}\phantom{$\blacktriangledown$} &      \textbf{0.0063$\pm$0.0}\phantom{$\blacktriangledown$} \\
       12 &  \underline{0.0305$\pm$0.01}\phantom{$\blacktriangledown$} &     \textbf{0.0271$\pm$0.01}\phantom{$\blacktriangledown$} \\
       23 &           0.4816$\pm$0.03{\color{red}$\blacktriangledown$} &     \textbf{0.4379$\pm$0.03}\phantom{$\blacktriangledown$} \\
       31 &              0.2467$\pm$0.02\phantom{$\blacktriangledown$} &      \textbf{0.245$\pm$0.02}\phantom{$\blacktriangledown$} \\
       54 &     \textbf{0.1694$\pm$0.03}\phantom{$\blacktriangledown$} &  \underline{0.1706$\pm$0.03}\phantom{$\blacktriangledown$} \\
      181 &  \underline{0.4014$\pm$0.04}\phantom{$\blacktriangledown$} &      \textbf{0.388$\pm$0.05}\phantom{$\blacktriangledown$} \\
      188 &  \underline{0.3432$\pm$0.05}\phantom{$\blacktriangledown$} &     \textbf{0.3393$\pm$0.04}\phantom{$\blacktriangledown$} \\
     1049 &              0.0877$\pm$0.01\phantom{$\blacktriangledown$} &     \textbf{0.0832$\pm$0.01}\phantom{$\blacktriangledown$} \\
     1067 &     \textbf{0.1483$\pm$0.01}\phantom{$\blacktriangledown$} &              0.1488$\pm$0.01\phantom{$\blacktriangledown$} \\
     1111 &      \textbf{0.0178$\pm$0.0}\phantom{$\blacktriangledown$} &                  nan$\pm$nan\phantom{$\blacktriangledown$} \\
     1457 &           0.2507$\pm$0.03{\color{red}$\blacktriangledown$} &       \textbf{0.24$\pm$0.04}\phantom{$\blacktriangledown$} \\
     1461 &               0.0995$\pm$0.0\phantom{$\blacktriangledown$} &      \textbf{0.0972$\pm$0.0}\phantom{$\blacktriangledown$} \\
     1464 &             0.22$\pm$0.03{\color{red}$\blacktriangledown$} &     \textbf{0.2067$\pm$0.02}\phantom{$\blacktriangledown$} \\
     1468 &     \textbf{0.0537$\pm$0.01}\phantom{$\blacktriangledown$} &  \underline{0.0556$\pm$0.02}\phantom{$\blacktriangledown$} \\
     1475 &            0.409$\pm$0.02{\color{red}$\blacktriangledown$} &     \textbf{0.3807$\pm$0.02}\phantom{$\blacktriangledown$} \\
     1485 &    \textbf{0.1062$\pm$0.01}{\color{green}$\blacktriangle$} &              0.2205$\pm$0.03\phantom{$\blacktriangledown$} \\
     1486 &     \textbf{0.0386$\pm$0.01}\phantom{$\blacktriangledown$} &              0.0479$\pm$0.01\phantom{$\blacktriangledown$} \\
     1487 &  \underline{0.0601$\pm$0.01}\phantom{$\blacktriangledown$} &     \textbf{0.0593$\pm$0.01}\phantom{$\blacktriangledown$} \\
     1489 &     \textbf{0.0863$\pm$0.01}\phantom{$\blacktriangledown$} &              0.0942$\pm$0.02\phantom{$\blacktriangledown$} \\
     1494 &     \textbf{0.1267$\pm$0.03}\phantom{$\blacktriangledown$} &              0.1349$\pm$0.02\phantom{$\blacktriangledown$} \\
     1515 &     \textbf{0.1298$\pm$0.04}\phantom{$\blacktriangledown$} &  \underline{0.1316$\pm$0.03}\phantom{$\blacktriangledown$} \\
     1590 &                0.148$\pm$0.0\phantom{$\blacktriangledown$} &     \textbf{0.1448$\pm$0.01}\phantom{$\blacktriangledown$} \\
     4134 &           0.2293$\pm$0.01{\color{red}$\blacktriangledown$} &     \textbf{0.2058$\pm$0.02}\phantom{$\blacktriangledown$} \\
     4135 &                  nan$\pm$nan\phantom{$\blacktriangledown$} &      \textbf{0.0584$\pm$0.0}\phantom{$\blacktriangledown$} \\
     4534 &  \underline{0.0345$\pm$0.01}\phantom{$\blacktriangledown$} &     \textbf{0.0304$\pm$0.01}\phantom{$\blacktriangledown$} \\
     4538 &           0.3509$\pm$0.02{\color{red}$\blacktriangledown$} &     \textbf{0.3173$\pm$0.01}\phantom{$\blacktriangledown$} \\
     4541 &               0.4359$\pm$0.0\phantom{$\blacktriangledown$} &     \textbf{0.4344$\pm$0.02}\phantom{$\blacktriangledown$} \\
    23512 &                  nan$\pm$nan\phantom{$\blacktriangledown$} &     \textbf{0.2984$\pm$0.01}\phantom{$\blacktriangledown$} \\
    23517 &               0.4862$\pm$0.0\phantom{$\blacktriangledown$} &     \textbf{0.4795$\pm$0.01}\phantom{$\blacktriangledown$} \\
    40498 &     \textbf{0.3273$\pm$0.01}\phantom{$\blacktriangledown$} &                  nan$\pm$nan\phantom{$\blacktriangledown$} \\
    40668 &                  nan$\pm$nan\phantom{$\blacktriangledown$} &     \textbf{0.1881$\pm$0.01}\phantom{$\blacktriangledown$} \\
    40670 &     \textbf{0.0483$\pm$0.01}\phantom{$\blacktriangledown$} &              0.0491$\pm$0.01\phantom{$\blacktriangledown$} \\
    40685 &               0.0009$\pm$0.0\phantom{$\blacktriangledown$} &      \textbf{0.0005$\pm$0.0}\phantom{$\blacktriangledown$} \\
    40701 &     \textbf{0.0464$\pm$0.01}\phantom{$\blacktriangledown$} &               0.047$\pm$0.01\phantom{$\blacktriangledown$} \\
    40900 &      \textbf{0.0078$\pm$0.0}\phantom{$\blacktriangledown$} &                  nan$\pm$nan\phantom{$\blacktriangledown$} \\
    40975 &      \textbf{0.004$\pm$0.0}{\color{green}$\blacktriangle$} &  \underline{0.0141$\pm$0.02}\phantom{$\blacktriangledown$} \\
    40978 &     \textbf{0.0305$\pm$0.01}\phantom{$\blacktriangledown$} &   \underline{0.0328$\pm$0.0}\phantom{$\blacktriangledown$} \\
    40981 &     \textbf{0.1348$\pm$0.03}\phantom{$\blacktriangledown$} &              0.1449$\pm$0.04\phantom{$\blacktriangledown$} \\
    40982 &           0.2485$\pm$0.03{\color{red}$\blacktriangledown$} &     \textbf{0.1881$\pm$0.01}\phantom{$\blacktriangledown$} \\
    40983 &              0.0176$\pm$0.01\phantom{$\blacktriangledown$} &       \textbf{0.015$\pm$0.0}\phantom{$\blacktriangledown$} \\
    40984 &     \textbf{0.0277$\pm$0.01}\phantom{$\blacktriangledown$} &               0.0303$\pm$0.0\phantom{$\blacktriangledown$} \\
    40996 &                  nan$\pm$nan\phantom{$\blacktriangledown$} &      \textbf{0.1364$\pm$0.0}\phantom{$\blacktriangledown$} \\
    41027 &    \textbf{0.1519$\pm$0.01}{\color{green}$\blacktriangle$} &              0.1635$\pm$0.01\phantom{$\blacktriangledown$} \\
    41138 &               0.0102$\pm$0.0\phantom{$\blacktriangledown$} &      \textbf{0.0093$\pm$0.0}\phantom{$\blacktriangledown$} \\
    41142 &     \textbf{0.2707$\pm$0.02}\phantom{$\blacktriangledown$} &              0.2786$\pm$0.01\phantom{$\blacktriangledown$} \\
    41143 &               0.197$\pm$0.02\phantom{$\blacktriangledown$} &      \textbf{0.1963$\pm$0.0}\phantom{$\blacktriangledown$} \\
    41144 &    \textbf{0.0898$\pm$0.01}{\color{green}$\blacktriangle$} &               0.2484$\pm$0.0\phantom{$\blacktriangledown$} \\
    41145 &    \textbf{0.1611$\pm$0.03}{\color{green}$\blacktriangle$} &               0.2521$\pm$0.0\phantom{$\blacktriangledown$} \\
    41146 &    \textbf{0.0424$\pm$0.01}{\color{green}$\blacktriangle$} &               0.0697$\pm$0.0\phantom{$\blacktriangledown$} \\
    41147 &     \textbf{0.3336$\pm$0.0}{\color{green}$\blacktriangle$} &                  0.5$\pm$0.0\phantom{$\blacktriangledown$} \\
    41150 &                  nan$\pm$nan\phantom{$\blacktriangledown$} &      \textbf{0.0902$\pm$0.0}\phantom{$\blacktriangledown$} \\
    41156 &              0.1554$\pm$0.02\phantom{$\blacktriangledown$} &      \textbf{0.147$\pm$0.02}\phantom{$\blacktriangledown$} \\
    41157 &              0.28$\pm$0.1{\color{red}$\blacktriangledown$} &         \textbf{0.1$\pm$0.0}\phantom{$\blacktriangledown$} \\
    41158 &     \textbf{0.0597$\pm$0.01}\phantom{$\blacktriangledown$} &              0.0683$\pm$0.01\phantom{$\blacktriangledown$} \\
    41159 &    \textbf{0.1768$\pm$0.01}{\color{green}$\blacktriangle$} &               0.2078$\pm$0.0\phantom{$\blacktriangledown$} \\
    41161 &      \textbf{0.004$\pm$0.0}{\color{green}$\blacktriangle$} &               0.0265$\pm$0.0\phantom{$\blacktriangledown$} \\
    41162 &     \textbf{0.1026$\pm$0.0}{\color{green}$\blacktriangle$} &              0.1149$\pm$0.02\phantom{$\blacktriangledown$} \\
    41163 &    \textbf{0.0211$\pm$0.01}{\color{green}$\blacktriangle$} &                0.038$\pm$0.0\phantom{$\blacktriangledown$} \\
    41164 &     \textbf{0.333$\pm$0.02}{\color{green}$\blacktriangle$} &               0.3653$\pm$0.0\phantom{$\blacktriangledown$} \\
    41165 &     \textbf{0.6147$\pm$0.02}\phantom{$\blacktriangledown$} &                  nan$\pm$nan\phantom{$\blacktriangledown$} \\
    41166 &     \textbf{0.2889$\pm$0.03}\phantom{$\blacktriangledown$} &                  nan$\pm$nan\phantom{$\blacktriangledown$} \\
    41167 &                  nan$\pm$nan\phantom{$\blacktriangledown$} &      \textbf{0.9626$\pm$0.0}\phantom{$\blacktriangledown$} \\
    41168 &                  nan$\pm$nan\phantom{$\blacktriangledown$} &      \textbf{0.3407$\pm$0.0}\phantom{$\blacktriangledown$} \\
    41169 &    \textbf{0.6845$\pm$0.02}{\color{green}$\blacktriangle$} &               0.7263$\pm$0.0\phantom{$\blacktriangledown$} \\
    42732 &      \textbf{0.1217$\pm$0.0}\phantom{$\blacktriangledown$} &                  nan$\pm$nan\phantom{$\blacktriangledown$} \\
    42733 &      \textbf{0.1684$\pm$0.0}\phantom{$\blacktriangledown$} &                  nan$\pm$nan\phantom{$\blacktriangledown$} \\
    42734 &                  nan$\pm$nan\phantom{$\blacktriangledown$} &                  nan$\pm$nan\phantom{$\blacktriangledown$} \\
\bottomrule
\end{tabular}
